Deep learning for solution and inversion of structural mechanics and vibrations

Deep learning has been the most popular machine learning method in the last few years. In this chapter, we present the application of deep learning and physics-informed neural networks concerning structural mechanics and vibration problems. Demonstration problems involve de-noising data, solution to time-dependent ordinary and partial differential equations, and characterizing the system's response for a given data.

==> Preface.tex <==
\chapter*{Preface}
\label{Preface}


This set of files can be used to create your typescript in \LaTeX. You can add packages as necessary.

References need to be at the chapter level and you may find the package \href{http://www.ctan.org/pkg/chapterbib}{chapterbib} with the option [sectionbib] useful for this.   Include references at the end of each chapter with 
\begin{verbatim}
\bibliographystyle{unsrt}
\bibliography{filename}
\end{verbatim}
where `filename' is the name of your bib file containing the reference source information. Remember to bibtex every chapter-level aux file before final compilation.



==> Symbols.tex <==
\chapter*{Symbols}

% a list of symbols or a glossary are not essential and could also go in the back matter

\begin{tabbing}
12345\=\kill
$\alpha$ \> Temperature coefficient of linear expansion (K$^{-1}$)\\
$\beta$ \> Temperature coefficient of volume expansion (K$^{-1}$)\\
$\gamma $ \> Ratio of heat capacities \\
$\epsilon $ \> Permittivity\\
$\kappa$ \> Dielectric constant\\
$\lambda $ \> Wavelength (m)\\
$\rho $ \> Density (kg/m$^3$)\\
\textbf{B}   \>Magnetic field (T)\\
C \>Molar heat capacity (JKg$^{-1}$K$^{-1}$)\\
f \> Frequency\\
k \> Thermal conductivity (Wm$^{-1}$K$^{-1}$)\\
R  \> Ideal gas constant (8.31 Jmol$^{-1}$K$^{-1}$)\\

\end{tabbing}
